Physical properties of circumnuclear ionising clusters. III. Kinematics of gas and stars in NGC 7742

In this third paper of a series, we study the kinematics of the ionised gas and stars, calculating the dynamical masses of the circumnuclear star-forming regions in the ring of of the face-on spiral NGC 7742. We have used high spectral resolution data from the MEGARA instrument attached to the Gran Telescopio Canarias (GTC) to measure the kinematical components of the nebular emission lines of selected HII regions and the stellar velocity dispersions from the CaT absorption lines that allow the derivation of the associated cluster virialized masses. The emission line profiles show two different kinematical components: a narrow one with velocity dispersion $\sim$ 10 km/s and a broad one with velocity dispersion similar to those found for the stellar absorption lines. The derived star cluster dynamical masses range from 2.5 $\times$ 10$^6$ to 10.0 $\times$ 10$^7$ M$_\odot$. The comparison of gas and stellar velocity dispersions suggests a scenario where the clusters have formed simultaneously in a first star formation episode with a fraction of the stellar evolution feedback remaining trapped in the cluster, subject to the same gravitational potential as the cluster stars. Between 0.15 and 7.07 % of the total dynamical mass of the cluster would have cooled down and formed a new, younger, population of stars, responsible for the ionisation of the gas currently observed.

==> Tables/Sigma_MEGARA.tex <==
\begin{center}
\begin{longtable}{llllll}
\caption{Emmision line velocity dispersions in km/s.}\\
\hline
Region ID      & Component & \begin{tabular}[c]{@{}c@{}} $\sigma$(H$\alpha$) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} $\sigma$([NII]$\lambda$6584 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} $\sigma$([SII]$\lambda$6717 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} $\sigma$([SIII]$\lambda$9532 \AA) \\ (km/s)\end{tabular}
\\ \hline
\endfirsthead
\caption{continued.}\\
\hline
Region ID      & Component & \begin{tabular}[c]{@{}c@{}} $\sigma$(H$\alpha$) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} $\sigma$([NII]$\lambda$6584 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} $\sigma$([SII]$\lambda$6717 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} $\sigma$([SIII]$\lambda$9532 \AA) \\ (km/s)\end{tabular}
\\ \hline
\endhead
\hline
\endfoot
%%

R1 & Narrow & 10.29 $\pm$ 0.09 & 7.88 $\pm$ 0.15 & 12.41 $\pm$ 0.80 & 18.98 $\pm$ 0.53 \\
  & Broad & 19.60 $\pm$ 0.20 & 18.30 $\pm$ 0.28 & 40.22 $\pm$ 4.14 & 62.64 $\pm$ 6.50 \\ 
  & Aditional & 47.7 $\pm$ 1.1 & 48.30 $\pm$ 2.34 &  - &  - \\
\\
R3 & Narrow & 14.46 $\pm$ 0.08 & 12.67 $\pm$ 0.13 & 13.82 $\pm$ 0.65 & 13.68 $\pm$ 0.44 \\
  & Broad & 43.68 $\pm$ 1.66 & 34.51 $\pm$ 2.02 & 53.56 $\pm$ 8.84 &  - \\ 
\\
R4 & Narrow & 10.53 $\pm$ 0.12 & 12.44 $\pm$ 0.21 & 12.00 $\pm$ 1.34 & 14.06 $\pm$ 0.58 \\
  & Broad & 27.88 $\pm$ 0.59 & 45.04 $\pm$ 3.09 & 33.12 $\pm$ 3.54 &  - \\ 
  & Aditional & 69.2 $\pm$ 10.3 &  - &  - &  - \\
\\
R5 & Narrow & 11.95 $\pm$ 0.09 & 10.36 $\pm$ 0.14 & 15.29 $\pm$ 1.02 & 5.87 $\pm$ 0.12 \\
  & Broad & 30.27 $\pm$ 1.40 & 28.68 $\pm$ 1.95 &  - &  - \\ 
\\
R6 & Narrow & 11.75 $\pm$ 0.11 & 11.09 $\pm$ 0.19 & 12.89 $\pm$ 0.97 & 5.34 $\pm$ 0.17 \\
\\
R7 & Narrow & 10.35 $\pm$ 0.12 & 10.66 $\pm$ 0.24 & 17.71 $\pm$ 0.96 & 12.19 $\pm$ 0.59 \\
  & Broad & 34.20 $\pm$ 2.12 & 44.95 $\pm$ 7.76 &  - &  - \\ 
\\
R8 & Narrow & 11.07 $\pm$ 0.12 & 10.65 $\pm$ 0.24 & 20.54 $\pm$ 1.44 & 5.47 $\pm$ 0.19 \\
  & Broad & 40.85 $\pm$ 3.06 & 37.46 $\pm$ 4.33 &  - &  - \\ 
\\
R9 & Narrow & 11.41 $\pm$ 0.11 & 10.77 $\pm$ 0.18 & 13.59 $\pm$ 0.77 & 10.10 $\pm$ 0.25 \\
  & Broad & 34.60 $\pm$ 2.60 & 55.29 $\pm$ 13.54 &  - &  - \\ 
\\
R10 & Narrow & 9.37 $\pm$ 0.09 & 10.25 $\pm$ 0.19 & 14.87 $\pm$ 0.88 & 13.97 $\pm$ 0.59 \\
  & Broad & 25.02 $\pm$ 0.73 & 31.00 $\pm$ 2.90 &  - &  - \\ 
  & Aditional & 91.4 $\pm$ 47.2 &  - &  - &  - \\
\\
R11 & Narrow & 9.54 $\pm$ 0.08 & 8.20 $\pm$ 0.14 & 15.92 $\pm$ 0.94 & 10.16 $\pm$ 0.61 \\
  & Broad & 25.85 $\pm$ 0.68 & 27.36 $\pm$ 1.51 &  - &  - \\ 
\\
R12 & Narrow & 10.09 $\pm$ 0.14 & 12.29 $\pm$ 0.29 & 14.00 $\pm$ 0.90 & 10.74 $\pm$ 0.65 \\
  & Broad & 32.02 $\pm$ 1.49 & 63.10 $\pm$ 19.95 &  - &  - \\ 
\\
R14 & Narrow & 7.83 $\pm$ 0.07 & 8.97 $\pm$ 0.15 & 16.32 $\pm$ 0.88 & 20.11 $\pm$ 1.13 \\
  & Broad & 25.41 $\pm$ 0.79 & 41.01 $\pm$ 4.28 &  - &  - \\ 
\\
R15 & Narrow & 8.76 $\pm$ 0.10 & 7.97 $\pm$ 0.19 & 13.37 $\pm$ 0.99 & 18.32 $\pm$ 1.40 \\
  & Broad & 27.77 $\pm$ 1.86 & 24.11 $\pm$ 1.70 &  - &  - \\ 
\\
R16 & Narrow & 10.18 $\pm$ 0.07 & 10.38 $\pm$ 0.14 & 17.69 $\pm$ 0.58 & 12.26 $\pm$ 0.57 \\
  & Broad & 32.21 $\pm$ 1.18 & 38.31 $\pm$ 3.09 &  - &  - \\ 
\\
R17 & Narrow & 10.12 $\pm$ 0.13 & 11.85 $\pm$ 0.23 & 14.46 $\pm$ 0.87 & 10.94 $\pm$ 0.40 \\
  & Broad & 20.61 $\pm$ 0.66 & 67.10 $\pm$ 38.19 &  - &  - \\ 
  & Aditional & 56.2 $\pm$ 19.7 &  - &  - &  - \\
\\
R18 & Narrow & 9.77 $\pm$ 0.10 & 9.00 $\pm$ 0.16 & 12.35 $\pm$ 0.61 & 8.77 $\pm$ 0.44 \\
  & Broad & 21.93 $\pm$ 0.57 & 27.39 $\pm$ 1.72 &  - &  - \\ 
\\
R19 & Narrow & 10.56 $\pm$ 0.21 & 11.27 $\pm$ 0.40 & 20.29 $\pm$ 1.60 & 11.04 $\pm$ 0.80 \\
  & Broad & 28.58 $\pm$ 1.22 & 31.66 $\pm$ 4.27 &  - &  - \\ 
\\
R20 & Narrow & 9.46 $\pm$ 0.13 & 10.50 $\pm$ 0.26 & 15.92 $\pm$ 1.32 & 9.73 $\pm$ 0.49 \\
  & Broad & 28.46 $\pm$ 2.30 & 52.29 $\pm$ 21.03 &  - &  - \\ 
\\
R21 & Narrow & 10.71 $\pm$ 0.13 & 10.49 $\pm$ 0.22 & 18.39 $\pm$ 1.01 & 14.14 $\pm$ 1.27 \\
  & Broad & 32.84 $\pm$ 1.67 & 39.08 $\pm$ 4.47 &  - &  - \\ 
\\
R22 & Narrow & 10.31 $\pm$ 0.10 & 11.17 $\pm$ 0.21 & 20.41 $\pm$ 1.16 & 8.64 $\pm$ 0.51 \\
  & Broad & 26.64 $\pm$ 0.93 & 36.56 $\pm$ 3.88 &  - &  - \\ 
\\
R23 & Narrow & 9.31 $\pm$ 0.08 & 10.07 $\pm$ 0.17 & 15.81 $\pm$ 0.85 &  - \\ 
  & Broad & 26.19 $\pm$ 0.69 & 35.65 $\pm$ 3.30 &  - &  - \\ 
\\
R25 & Narrow & 6.98 $\pm$ 0.15 & 9.97 $\pm$ 0.36 & 9.66 $\pm$ 1.26 & 9.46 $\pm$ 0.68 \\
  & Broad & 29.94 $\pm$ 2.00 & 47.27 $\pm$ 20.12 &  - &  - \\ 
\\
R26 & Narrow & 10.41 $\pm$ 0.08 & 10.13 $\pm$ 0.16 & 14.80 $\pm$ 0.59 & 10.40 $\pm$ 0.42 \\
  & Broad & 30.04 $\pm$ 0.97 & 25.22 $\pm$ 1.37 &  - &  - \\ 
\\
R27 & Narrow & 9.94 $\pm$ 0.11 & 9.47 $\pm$ 0.19 & 14.73 $\pm$ 1.32 & 6.12 $\pm$ 0.33 \\
  & Broad & 31.70 $\pm$ 3.32 & 47.44 $\pm$ 12.08 &  - &  - \\ 
\\
R28 & Narrow & 8.99 $\pm$ 0.18 & 11.94 $\pm$ 0.50 & 7.64 $\pm$ 1.18 & 16.24 $\pm$ 1.24 \\
  & Broad & 31.40 $\pm$ 2.45 & 38.83 $\pm$ 12.25 &  - &  - \\ 
\\
R29 & Narrow & 9.72 $\pm$ 0.13 & 10.03 $\pm$ 0.32 & 23.05 $\pm$ 2.16 &  - \\ 
  & Broad & 46.27 $\pm$ 5.53 & 50.99 $\pm$ 14.53 &  - &  - \\ 
\\
R30 & Narrow & 6.12 $\pm$ 0.10 & 6.80 $\pm$ 0.20 & 12.79 $\pm$ 1.29 & 11.74 $\pm$ 0.95 \\
  & Broad & 22.06 $\pm$ 1.27 & 23.59 $\pm$ 2.72 &  - &  - \\ 
\\
R31 & Narrow & 10.36 $\pm$ 0.14 & 10.80 $\pm$ 0.24 & 18.52 $\pm$ 1.04 & 17.96 $\pm$ 2.12 \\
  & Broad & 30.33 $\pm$ 1.45 & 46.99 $\pm$ 5.77 &  - &  - \\ 
\\
R32 & Narrow & 8.48 $\pm$ 0.21 & 6.86 $\pm$ 0.33 & 15.81 $\pm$ 2.74 & 3.67 $\pm$ 0.44 \\
  & Broad & 35.29 $\pm$ 6.62 & 27.44 $\pm$ 10.01 &  - &  - \\ 
\\
R33 & Narrow & 7.66 $\pm$ 0.09 & 8.41 $\pm$ 0.18 & 13.81 $\pm$ 0.79 &  - \\ 
  & Broad & 24.64 $\pm$ 1.01 & 29.96 $\pm$ 2.83 &  - &  - \\ 
\\
R34 & Narrow & 4.95 $\pm$ 0.15 & 13.44 $\pm$ 0.52 & 17.72 $\pm$ 2.15 & 4.98 $\pm$ 0.44 \\
  & Broad & 20.81 $\pm$ 0.90 &  - &  - &  - \\ 
\\
R35 & Narrow & 9.20 $\pm$ 0.14 & 9.53 $\pm$ 0.28 & 12.83 $\pm$ 1.01 & 16.65 $\pm$ 1.03 \\
  & Broad & 34.45 $\pm$ 2.97 & 37.56 $\pm$ 6.46 &  - &  - \\ 
\\
R36 & Narrow & 7.68 $\pm$ 0.10 & 8.41 $\pm$ 0.21 & 14.11 $\pm$ 0.87 & 13.05 $\pm$ 0.98 \\
  & Broad & 25.87 $\pm$ 0.87 & 31.60 $\pm$ 2.78 &  - &  - \\ 
\\
R37 & Narrow & 10.09 $\pm$ 0.21 & 10.35 $\pm$ 0.42 & 11.40 $\pm$ 1.66 &  - \\ 
  & Broad & 31.68 $\pm$ 2.72 & 40.25 $\pm$ 8.20 &  - &  - \\ 
\\
R38 & Narrow & 6.97 $\pm$ 0.10 & 4.21 $\pm$ 0.19 & 12.62 $\pm$ 1.00 &  - \\ 
  & Broad & 23.90 $\pm$ 1.51 & 16.62 $\pm$ 0.74 &  - &  - \\ 
\\
R41 & Narrow & 11.91 $\pm$ 0.12 & 12.55 $\pm$ 0.25 & 18.88 $\pm$ 1.07 & 18.31 $\pm$ 1.41 \\
  & Broad & 41.70 $\pm$ 3.34 & 60.96 $\pm$ 10.48 &  - &  - \\ 
\\
R42 & Narrow & 11.13 $\pm$ 0.10 & 10.37 $\pm$ 0.18 & 14.25 $\pm$ 0.90 &  - \\ 
  & Broad & 30.96 $\pm$ 2.51 & 42.24 $\pm$ 8.52 &  - &  - \\ 
\\
R43 & Narrow & 11.55 $\pm$ 0.16 & 10.64 $\pm$ 0.30 & 12.69 $\pm$ 0.85 & 14.99 $\pm$ 1.45 \\
  & Broad & 29.91 $\pm$ 2.93 & 46.25 $\pm$ 12.56 &  - &  - \\ 
\\
R44 & Narrow & 10.43 $\pm$ 0.21 & 9.06 $\pm$ 0.35 & 15.51 $\pm$ 1.14 & 27.95 $\pm$ 3.84 \\
  & Broad & 36.42 $\pm$ 4.41 & 26.70 $\pm$ 3.23 &  - &  - \\ 
\\
R45 & Narrow & 9.50 $\pm$ 0.14 & 10.45 $\pm$ 0.38 & 17.98 $\pm$ 1.47 & 21.76 $\pm$ 5.07 \\
  & Broad & 28.71 $\pm$ 1.82 & 43.38 $\pm$ 6.65 &  - &  - \\ 
\\
R48 & Narrow & 8.18 $\pm$ 0.19 & 13.34 $\pm$ 0.54 & 16.93 $\pm$ 1.30 & 17.43 $\pm$ 4.00 \\
\\
R50 & Narrow & 12.32 $\pm$ 0.14 & 11.97 $\pm$ 0.28 & 18.73 $\pm$ 1.03 &  - \\ 
  & Broad & 33.93 $\pm$ 1.99 & 30.08 $\pm$ 2.95 &  - &  - \\ 
\\
R51 & Narrow & 7.05 $\pm$ 0.19 & 6.25 $\pm$ 0.41 & 16.80 $\pm$ 1.57 &  - \\ 
  & Broad & 20.33 $\pm$ 1.34 & 26.24 $\pm$ 2.72 &  - &  - \\ 
  & Aditional & 139.6 $\pm$ 76.2 &  - &  - &  - \\
\\
R52 & Narrow & 8.57 $\pm$ 0.11 & 11.37 $\pm$ 0.29 & 17.03 $\pm$ 1.06 &  - \\ 
  & Broad & 25.61 $\pm$ 0.94 & 56.11 $\pm$ 9.65 &  - &  - \\ 
\\
R53 & Narrow & 10.07 $\pm$ 0.19 & 10.89 $\pm$ 0.32 & 13.81 $\pm$ 1.01 & 15.46 $\pm$ 1.20 \\
  & Broad & 26.34 $\pm$ 1.96 & 65.51 $\pm$ 23.35 &  - &  - \\ 
\\
R54 & Narrow & 7.88 $\pm$ 0.25 & 9.99 $\pm$ 0.63 & 16.48 $\pm$ 1.59 & 48.95 $\pm$ 21.75 \\
  & Broad & 25.72 $\pm$ 1.54 & 39.64 $\pm$ 5.50 &  - &  - \\ 
\\
R55 & Narrow & 10.27 $\pm$ 0.20 & 15.42 $\pm$ 0.56 & 14.52 $\pm$ 1.18 & 22.84 $\pm$ 3.33 \\
  & Broad & 25.14 $\pm$ 1.85 &  - &  - &  - \\ 
\\
R56 & Narrow & 8.12 $\pm$ 0.15 & 10.99 $\pm$ 0.39 & 15.00 $\pm$ 1.43 &  - \\ 
  & Broad & 29.55 $\pm$ 1.89 & 61.53 $\pm$ 21.19 &  - &  - \\ 
\\
R57 & Narrow & 10.86 $\pm$ 0.22 & 15.50 $\pm$ 0.47 & 20.19 $\pm$ 1.41 & 21.58 $\pm$ 2.17 \\
  & Broad & 27.27 $\pm$ 1.48 &  - &  - &  - \\ 
\\
R58 & Narrow & 7.78 $\pm$ 0.17 & 7.73 $\pm$ 0.34 & 12.98 $\pm$ 1.13 & 1.96 $\pm$ 0.17 \\
  & Broad & 20.68 $\pm$ 0.78 & 19.72 $\pm$ 1.37 &  - &  - \\ 
\\
R59 & Narrow & 7.75 $\pm$ 0.22 & 7.53 $\pm$ 0.36 & 14.92 $\pm$ 1.13 & 20.25 $\pm$ 2.36 \\
  & Broad & 19.60 $\pm$ 0.56 & 21.82 $\pm$ 1.41 &  - &  - \\ 
\\
R60 & Narrow & 7.11 $\pm$ 0.25 & 9.97 $\pm$ 0.38 & 19.17 $\pm$ 2.03 &  - \\ 
  & Broad & 16.61 $\pm$ 0.56 & 46.88 $\pm$ 10.37 &  - &  - \\ 
  & Aditional & 53.9 $\pm$ 16.5 &  - &  - &  - \\
\\
R61 & Narrow & 9.62 $\pm$ 0.24 & 11.16 $\pm$ 0.45 & 11.74 $\pm$ 1.50 &  - \\ 
  & Broad & 27.83 $\pm$ 2.18 & 73.67 $\pm$ 27.62 &  - &  - \\ 
\\
R62 & Narrow & 9.01 $\pm$ 0.19 & 8.64 $\pm$ 0.37 & 6.62 $\pm$ 0.85 & 6.74 $\pm$ 0.57 \\
  & Broad & 73.66 $\pm$ 21.55 & 50.73 $\pm$ 14.11 &  - &  - \\ 
\\
R63 & Narrow & 9.47 $\pm$ 0.21 & 12.55 $\pm$ 0.53 & 15.19 $\pm$ 1.37 & 31.98 $\pm$ 6.23 \\
  & Broad & 25.75 $\pm$ 3.31 &  - &  - &  - \\ 
\\
R64 & Narrow & 3.11 $\pm$ 0.07 & 9.11 $\pm$ 0.35 & 16.11 $\pm$ 4.13 &  - \\ 
  & Broad & 21.80 $\pm$ 1.04 & 36.57 $\pm$ 7.47 &  - &  - \\ 
\\
R65 & Narrow & 10.79 $\pm$ 0.30 & 13.66 $\pm$ 1.03 & 20.31 $\pm$ 2.44 &  - \\ 
  & Broad & 16.04 $\pm$ 2.95 & 43.69 $\pm$ 10.07 &  - &  - \\ 
\\
R66 & Narrow & 12.53 $\pm$ 0.71 & 20.60 $\pm$ 2.26 & 25.61 $\pm$ 4.07 &  - \\ 
  & Broad & 62.39 $\pm$ 16.46 &  - &  - &  - \\ 
\\
R67 & Narrow & 8.64 $\pm$ 0.25 & 13.89 $\pm$ 0.61 & 20.49 $\pm$ 2.21 &  - \\ 
  & Broad & 24.97 $\pm$ 1.97 &  - &  - &  - \\ 
  & Aditional & 107.1 $\pm$ 60.4 &  - &  - &  - \\
\\
R69 & Narrow & 2.36 $\pm$ 0.09 & 15.15 $\pm$ 0.82 & 8.55 $\pm$ 1.11 &  - \\ 
  & Broad & 18.65 $\pm$ 0.86 &  - &  - &  - \\ 
\\
R70 & Narrow & 6.80 $\pm$ 0.20 & 9.11 $\pm$ 0.49 & 21.58 $\pm$ 2.33 & 14.70 $\pm$ 2.17 \\
  & Broad & 27.54 $\pm$ 1.71 & 39.91 $\pm$ 5.20 &  - &  - \\ 
\\
R71 & Narrow & 6.30 $\pm$ 0.31 & - & 26.32 $\pm$ 3.93 & 30.00 $\pm$ 8.37 \\
  & Broad & 27.08 $\pm$ 2.36 & 27.03 $\pm$ 3.31 &  - &  - \\ 
\\
R72 & Narrow & 8.42 $\pm$ 0.46 & 7.45 $\pm$ 0.75 & 5.52 $\pm$ 1.11 & 28.71 $\pm$ 8.92 \\
  & Broad & 37.55 $\pm$ 13.56 &  - &  - &  - \\ 
\\
R73 & Narrow & 7.44 $\pm$ 0.22 & 11.12 $\pm$ 0.50 & 18.87 $\pm$ 3.13 &  - \\ 
  & Broad & 23.58 $\pm$ 2.39 &  - &  - &  - \\ 
\\
R74 & Narrow & 3.88 $\pm$ 0.19 & 12.69 $\pm$ 0.55 & 20.64 $\pm$ 2.43 &  - \\ 
  & Broad & 18.01 $\pm$ 0.72 &  - &  - &  - \\ 
\\
R75 & Narrow & 6.27 $\pm$ 0.23 & 8.96 $\pm$ 0.56 & 16.42 $\pm$ 1.94 & 30.85 $\pm$ 16.07 \\
  & Broad & 24.80 $\pm$ 1.23 & 33.70 $\pm$ 4.61 &  - &  - \\ 
\\
R76 & Narrow & 1.38 $\pm$ 0.11 & 11.82 $\pm$ 1.16 &  - &  - \\ 
  & Broad & 23.41 $\pm$ 3.21 &  - &  - &  - \\ 
\\
R77 & Narrow & 12.34 $\pm$ 0.64 & 11.89 $\pm$ 1.32 & 17.13 $\pm$ 2.58 & 14.31 $\pm$ 4.20 \\
  & Broad & 14.85 $\pm$ 3.35 & 41.70 $\pm$ 10.83 &  - &  - \\ 
\\
R78 & Narrow & 14.61 $\pm$ 0.42 & 14.73 $\pm$ 1.01 & 19.33 $\pm$ 2.00 &  - \\ 
\\
R79 & Narrow & 14.24 $\pm$ 0.43 & 14.83 $\pm$ 1.09 & 12.96 $\pm$ 1.79 &  - \\ 
\\
R80 & Narrow & 8.31 $\pm$ 0.56 & 20.28 $\pm$ 3.05 & 13.39 $\pm$ 2.68 & 25.07 $\pm$ 8.35 \\
  & Broad & 29.48 $\pm$ 5.07 &  - &  - &  - \\ 
\\
R81 & Narrow & 10.49 $\pm$ 0.38 & 13.53 $\pm$ 1.07 & 12.32 $\pm$ 3.04 & 15.98 $\pm$ 5.06 \\
\\
R83 & Narrow & 2.67 $\pm$ 0.14 & 15.04 $\pm$ 1.03 & 11.39 $\pm$ 2.37 & 16.80 $\pm$ 4.93 \\
  & Broad & 21.92 $\pm$ 1.62 &  - &  - &  - \\ 
\\
R84 & Narrow & 13.88 $\pm$ 0.53 & 15.14 $\pm$ 1.13 & 12.03 $\pm$ 3.18 &  - \\ 
\\
R85 & Narrow & 10.46 $\pm$ 0.39 & 18.51 $\pm$ 1.42 & 16.01 $\pm$ 2.57 &  - \\ 
\\
R86 & Narrow & 6.13 $\pm$ 0.43 & 6.36 $\pm$ 0.99 & 34.38 $\pm$ 5.99 & 34.37 $\pm$ 8.38 \\
  & Broad & 31.72 $\pm$ 7.24 & 35.05 $\pm$ 11.08 &  - &  - \\ 
  & Broad & 20.82 $\pm$ 4.51 & 9.20 $\pm$ 3.17 &  - &  - \\ 
\\
R88 & Narrow & 17.89 $\pm$ 0.87 & 17.76 $\pm$ 1.67 & 14.69 $\pm$ 2.73 &  - \\ 

\end{longtable}

\end{center}





==> Tables/Sigma_MEGARA_simple.tex <==
\begin{table*}
\centering
\caption{Emission line velocity dispersions in km/s.}
\label{tab:sigma_MEGARA}
\begin{tabular}{cccccc}
\hline
Region ID      & Component & \begin{tabular}[c]{@{}c@{}} $\sigma$(H$\alpha$) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} $\sigma$([NII]$\lambda$6584 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} $\sigma$([SII]$\lambda$6717 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} $\sigma$([SIII]$\lambda$9532 \AA) \\ (km/s)\end{tabular}
\\ \hline

R1 & Narrow & 10.29 $\pm$ 0.09 & 7.88 $\pm$ 0.15 & 12.41 $\pm$ 0.80 & 18.98 $\pm$ 0.53 \\
  & Broad & 19.60 $\pm$ 0.20 & 18.30 $\pm$ 0.28 & 40.22 $\pm$ 4.14 & 62.64 $\pm$ 6.50 \\ 
  & Aditional & 47.7 $\pm$ 1.1 & 48.30 $\pm$ 2.34 &  - &  - \\
\\
R3 & Narrow & 14.46 $\pm$ 0.08 & 12.67 $\pm$ 0.13 & 13.82 $\pm$ 0.65 & 13.68 $\pm$ 0.44 \\
  & Broad & 43.68 $\pm$ 1.66 & 34.51 $\pm$ 2.02 & 53.56 $\pm$ 8.84 &  - \\ 
\\
R4 & Narrow & 10.53 $\pm$ 0.12 & 12.44 $\pm$ 0.21 & 12.00 $\pm$ 1.34 & 14.06 $\pm$ 0.58 \\
  & Broad & 27.88 $\pm$ 0.59 & 45.04 $\pm$ 3.09 & 33.12 $\pm$ 3.54 &  - \\ 
  & Aditional & 69.2 $\pm$ 10.3 &  - &  - &  - \\
\hline


\end{tabular}
\tablefoot{
The complete table is available online; here only a part is shown as an example.
}
\end{table*}

==> Tables/Tabla_masas_din_MEGARA.tex <==


\begin{table}
\centering
\setlength{\tabcolsep}{3pt}
\caption{Stellar cluster masses and sizes for observed CNSFRs.}
\label{tab:mdyn_MEGARA}
\begin{tabular}{ccccc}
\hline
\begin{tabular}[c]{@{}c@{}}Region \\ ID\end{tabular} & N$_{knots}$ & \begin{tabular}[c]{@{}c@{}}R$^* _{mean}$ \\ (pc/knot)\end{tabular} 
& \begin{tabular}[c]{@{}c@{}} M$_{dyn}$ \\ (M$_\odot$)\end{tabular} & \begin{tabular}[c]{@{}c@{}} M$_{ion}$/M$_{dyn}$ \\ (per cent)\end{tabular} \\
\hline

R1 & 1 & 13.9 & (6.2 $\pm$ 3.6) $\times$ 10$^{6}$ & 2.57\\ 
R3 & 2 & 15.0 & (25.9 $\pm$ 2.7) $\times$ 10$^{6}$ & 1.47\\ 
R5 & 1 & 16.3 & (84.6 $\pm$ 3.0) $\times$ 10$^{6}$ & 0.15\\ 
R7 & 1 & 9.9 & (3.5 $\pm$ 1.5) $\times$ 10$^{6}$ & 6.61\\ 
R8 & 1 & 20.1 & (2.5 $\pm$ 2.6) $\times$ 10$^{7}$ & 1.32\\ 
R14 & 2 & 12.8 & (8.3 $\pm$ 2.0) $\times$ 10$^{6}$ & 2.20\\ 
R15 & 1 & 12.1 & (8.2 $\pm$ 3.9) $\times$ 10$^{6}$ & 1.45\\ 
R16 & 1 & 10.1 & (22.8 $\pm$ 3.6) $\times$ 10$^{6}$ & 2.26\\ 
R22 & 1 & 10.1 & (12.2 $\pm$ 6.5) $\times$ 10$^{6}$ & 2.24\\ 
R23 & 2 & 14.6 & (38.3 $\pm$ 8.6) $\times$ 10$^{6}$ & 0.73\\ 
R26 & 2 & 14.6 & (9.5 $\pm$ 2.3) $\times$ 10$^{6}$ & 3.00\\ 
R31 & 4 & 10.1 & (74.4 $\pm$ 7.6) $\times$ 10$^{6}$ & 0.40\\ 
R33 & 1 & 15.2 & (30.2 $\pm$ 6.8) $\times$ 10$^{6}$ & 0.77\\ 
R36 & 1 & 10.6 & (481.8 $\pm$ 6.6) $\times$ 10$^{5}$ & 0.77\\ 
R41 & 3 & 14.8 & (100.4 $\pm$ 6.7) $\times$ 10$^{6}$ & 0.59\\ 
R45 & 2 & 18.1 & (10.0 $\pm$ 2.3) $\times$ 10$^{7}$ & 0.19\\ 
R47 & 2 & 12.2 & (3.2 $\pm$ 1.1) $\times$ 10$^{7}$ & 0.55\\ 
R50 & 1 & 10.1 & (17.6 $\pm$ 3.9) $\times$ 10$^{6}$ & 1.21\\ 
R51 & 1 & 71.3 & (8.4 $\pm$ 3.1) $\times$ 10$^{7}$ & 0.39\\ 
R52 & 3 & 14.9 & (31.4 $\pm$ 4.9) $\times$ 10$^{6}$ & 1.46\\ 
R53 & 1 & 10.1 & (22.6 $\pm$ 1.0) $\times$ 10$^{6}$ & 0.58\\ 
R55 & 3 & 14.1 & (73.4 $\pm$ 6.7) $\times$ 10$^{6}$ & 0.13\\ 
R57 & 2 & 14.7 & (5.4 $\pm$ 1.1) $\times$ 10$^{6}$ & 7.07\\ 
R60 & 1 & 13.1 & (12.7 $\pm$ 5.8) $\times$ 10$^{6}$ & 0.90\\ 
R63 & 1 & 10.1 & (9.6 $\pm$ 4.3) $\times$ 10$^{6}$ & 1.33\\ 
R69 & 1 & 14.4 & (2.5 $\pm$ 2.4) $\times$ 10$^{6}$ & 4.16\\ 
R74 & 1 & 19.2 & (9.3 $\pm$ 4.6) $\times$ 10$^{6}$ & 1.14\\ 


\hline
\end{tabular}
\end{table}

==> Tables/Tabla_sigma_stars.tex <==


\begin{table}
\centering
\caption{Stellar cluster velocity dispersions in units of km/s.}
\label{tab:sigma_Stars_MEGARA}
\begin{tabular}{cc}
\hline
Region ID &  \begin{tabular}[c]{@{}c@{}} $\sigma_*$(CaT) \\ (km/s)\end{tabular}\\
\hline
R1 & 22.61 $\pm$ 6.65 \\
R3 & 31.43 $\pm$ 4.68 \\
R5 & 77.08 $\pm$ 1.37 \\
R7 & 20.19 $\pm$ 4.39 \\
R8 & 37.75 $\pm$ 19.32 \\
R14 & 19.34 $\pm$ 5.87 \\
R15 & 27.88 $\pm$ 6.61 \\
R16 & 50.82 $\pm$ 3.95 \\
R22 & 37.10 $\pm$ 9.98 \\
R23 & 38.75 $\pm$ 8.66 \\
R26 & 19.26 $\pm$ 6.86 \\
R31 & 45.87 $\pm$ 9.38 \\
R33 & 47.73 $\pm$ 5.41 \\
R36 & 72.04 $\pm$ 0.49 \\
R41 & 50.82 $\pm$ 4.95 \\
R45 & 56.26 $\pm$ 14.67 \\
R47 & 38.95 $\pm$ 13.01 \\
R50 & 44.64 $\pm$ 4.94 \\
R51 & 36.78 $\pm$ 6.83 \\
R52 & 28.40 $\pm$ 9.85 \\
R53 & 50.53 $\pm$ 1.13 \\
R55 & 44.67 $\pm$ 7.63 \\
R57 & 14.46 $\pm$ 4.49 \\
R60 & 33.36 $\pm$ 7.53 \\
R63 & 32.93 $\pm$ 7.31 \\
R69 & 14.25 $\pm$ 6.79 \\
R72 & 26.40 $\pm$ 4.24 \\
R74 & 23.56 $\pm$ 5.80 \\
R75 & 43.76 $\pm$ 6.35 \\
R88 & 20.65 $\pm$ 3.52 \\
\hline
\end{tabular}
\end{table}

==> Tables/Tabla_targets.tex <==
\begin{table*}
\centering
\caption{Target observations.}
\label{tab:targets}
\begin{tabular}{ccccccc}
\hline
Target      & \begin{tabular}[c]{@{}c@{}}RA \\ (hh:mm:ss.ss)\end{tabular}& \begin{tabular}[c]{@{}c@{}}DEC \\ (dd:mm:ss.ss)\end{tabular} &\begin{tabular}[c]{@{}c@{}}Field of View \\ Position Angle$^a$ \\ (degrees)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Exp. Time$^b$ (s)\\ VPH863\_HR \end{tabular}  & \begin{tabular}[c]{@{}c@{}}Exp. Time$^b$ (s)\\ VPH890\_LR\end{tabular} & \begin{tabular}[c]{@{}c@{}}Exp. Time$^b$ (s)\\ VPH665\_HR\end{tabular}\\ \hline 
NGC7742\_P1 & 23:44:16.02 &	10:46:05.80 & 0 & 1050 & 450 & 684\\
NGC7742\_P2 & 23:44:15.28 & 10:46:06.40 & 0 & 1050 & - & 684\\
NGC7742\_P2 & 23:44:15.28 & 10:46:06.40 & 90 & 1050 & 450 & 342\\
NGC7742\_P3 & 23:44:16.02 & 10:45:55.60 & 0 & 1050 & 450 & 684\\
NGC7742\_P4 & 23:44:15.28 & 10:45:55.00 & 90 & 1050 & 450 & 342\\ \hline
\end{tabular}
\tablefoot{
$^a$ From North toward East. The orientation of 0 deg implies that the North is aligned with the short side and the East-West axis with the long side of the detector.
$^b$ Total target observed time without overheads.
}
\end{table*}

==> Tables/TableEW.tex <==
\begin{center}
\begin{longtable}{lll}
\caption{Equivalent widths of stellar absorption lines and velocity dispersions of the observed CNSFRs.}\\
\hline
Region ID & \begin{tabular}[c]{@{}c@{}} EW(CaII)$^a$ \\ (\AA)\end{tabular} & \begin{tabular}[c]{@{}c@{}} EW(MgI) \\ (\AA)\end{tabular} \\ \hline
\endfirsthead
\caption{continued.}\\
\hline
Region ID & \begin{tabular}[c]{@{}c@{}} EW(CaII)$^a$ \\ (\AA)\end{tabular} & \begin{tabular}[c]{@{}c@{}} EW(MgI) \\ (\AA)\end{tabular} \\ \hline
\endhead
\hline
\endfoot

R1 & 7.307 $\pm$ 0.264 & 1.686 $\pm$ 0.035  \\ 
R3 & 7.301 $\pm$ 0.278 & 2.329 $\pm$ 0.063  \\ 
R4 & 7.558 $\pm$ 0.303 & 1.868 $\pm$ 0.044  \\ 
R5 & 7.418 $\pm$ 0.338 & 2.147 $\pm$ 0.048  \\ 
R6 & 7.118 $\pm$ 0.318 & 2.141 $\pm$ 0.073  \\ 
R7 & 6.732 $\pm$ 0.339 & 1.972 $\pm$ 0.056  \\ 
R8 & 7.350 $\pm$ 0.299 & 2.156 $\pm$ 0.060  \\ 
R9 & 7.571 $\pm$ 0.346 & 2.013 $\pm$ 0.054  \\ 
R10 & 7.008 $\pm$ 0.297 & 1.987 $\pm$ 0.048  \\ 
R11 & 7.281 $\pm$ 0.211 & 2.840 $\pm$ 0.092  \\ 
R12 & 7.279 $\pm$ 0.304 & 2.377 $\pm$ 0.062  \\ 
R14 & 7.150 $\pm$ 0.288 & 2.474 $\pm$ 0.065  \\ 
R15 & 7.033 $\pm$ 0.384 & 2.308 $\pm$ 0.066  \\ 
R16 & 8.796 $\pm$ 0.328 & 2.230 $\pm$ 0.063  \\ 
R17 & 8.094 $\pm$ 0.283 & 1.911 $\pm$ 0.054  \\ 
R18 & 7.138 $\pm$ 0.351 & 2.322 $\pm$ 0.076  \\ 
R19 & 6.682 $\pm$ 0.279 & 2.105 $\pm$ 0.064  \\ 
R20 & 8.003 $\pm$ 0.363 & 2.292 $\pm$ 0.067  \\ 
R21 & 7.592 $\pm$ 0.343 & 2.677 $\pm$ 0.082  \\ 
R22 & 7.549 $\pm$ 0.224 & 2.905 $\pm$ 0.109  \\ 
R23 & 6.828 $\pm$ 0.257 & 2.773 $\pm$ 0.093  \\  
R25 & 7.429 $\pm$ 0.298 & 2.619 $\pm$ 0.078  \\ 
R26 & 7.350 $\pm$ 0.219 & 2.306 $\pm$ 0.063  \\ 
R27 & 8.381 $\pm$ 0.381 & 2.025 $\pm$ 0.064  \\ 
R28 & 7.490 $\pm$ 0.340 & 2.429 $\pm$ 0.083  \\ 
R29 & 7.267 $\pm$ 0.268 & 2.741 $\pm$ 0.082  \\ 
R30 & 7.277 $\pm$ 0.283 & 2.733 $\pm$ 0.088  \\ 
R31 & 6.737 $\pm$ 0.297 & 2.336 $\pm$ 0.083  \\ 
R32 & 7.288 $\pm$ 0.282 & 2.784 $\pm$ 0.100  \\ 
R33 & 7.050 $\pm$ 0.255 & 2.496 $\pm$ 0.079  \\ 
R34 & 7.029 $\pm$ 0.338 & 2.119 $\pm$ 0.087  \\ 
R35 & 6.148 $\pm$ 0.342 & 2.338 $\pm$ 0.079  \\ 
R36 & 7.320 $\pm$ 0.257 & 2.913 $\pm$ 0.099  \\ 
R37 & 8.513 $\pm$ 0.348 & 2.273 $\pm$ 0.077  \\ 
R38 & 6.462 $\pm$ 0.286 & 2.263 $\pm$ 0.078  \\ 
R41 & 7.412 $\pm$ 0.295 & 2.799 $\pm$ 0.089  \\ 
R42 & 6.753 $\pm$ 0.332 & 2.411 $\pm$ 0.070  \\ 
R43 & 7.127 $\pm$ 0.268 & 2.800 $\pm$ 0.089  \\ 
R44 & 7.775 $\pm$ 0.390 & 2.620 $\pm$ 0.079  \\ 
R45 & 7.637 $\pm$ 0.233 & 2.928 $\pm$ 0.101  \\ 
R47 & 6.918 $\pm$ 0.297 & 2.580 $\pm$ 0.084  \\ 
R48 & 6.770 $\pm$ 0.296 & 2.583 $\pm$ 0.096  \\ 
R50 & 7.659 $\pm$ 0.252 & 2.587 $\pm$ 0.082  \\ 
R51 & 7.489 $\pm$ 0.238 & 3.024 $\pm$ 0.118  \\ 
R52 & 6.840 $\pm$ 0.283 & 2.486 $\pm$ 0.081  \\ 
R53 & 7.125 $\pm$ 0.298 & 2.128 $\pm$ 0.075  \\ 
R54 & 6.640 $\pm$ 0.241 & 2.416 $\pm$ 0.080  \\ 
R55 & 7.522 $\pm$ 0.310 & 2.708 $\pm$ 0.100  \\ 
R56 & 6.720 $\pm$ 0.268 & 2.682 $\pm$ 0.082  \\ 
R57 & 6.945 $\pm$ 0.258 & 3.077 $\pm$ 0.120  \\ 
R58 & 7.636 $\pm$ 0.296 & 2.936 $\pm$ 0.104  \\ 
R59 & 8.311 $\pm$ 0.296 & 2.896 $\pm$ 0.112  \\ 
R60 & 6.606 $\pm$ 0.362 & 2.272 $\pm$ 0.068  \\ 
R61 & 8.889 $\pm$ 0.723 & 2.482 $\pm$ 0.080  \\ 
R62 & 7.057 $\pm$ 0.377 & 2.564 $\pm$ 0.092  \\ 
R63 & 8.640 $\pm$ 0.489 & 2.321 $\pm$ 0.077  \\ 
R64 & 6.857 $\pm$ 0.299 & 2.387 $\pm$ 0.068  \\ 
R65 & 7.876 $\pm$ 0.254 & 2.609 $\pm$ 0.080  \\ 
R66 & 7.559 $\pm$ 0.224 & 2.485 $\pm$ 0.084  \\ 
R67 & 9.055 $\pm$ 0.422 & 2.408 $\pm$ 0.076  \\ 
R69 & 6.696 $\pm$ 0.229 & 2.881 $\pm$ 0.108  \\ 
R70 & 7.076 $\pm$ 0.278 & 2.845 $\pm$ 0.111  \\ 
R71 & 6.958 $\pm$ 0.236 & 3.010 $\pm$ 0.106  \\ 
R72 & 7.296 $\pm$ 0.242 & 3.173 $\pm$ 0.131  \\ 
R73 & 6.577 $\pm$ 0.209 & 3.506 $\pm$ 0.166  \\ 
R74 & 6.576 $\pm$ 0.323 & 2.888 $\pm$ 0.114  \\ 
R75 & 6.743 $\pm$ 0.241 & 3.244 $\pm$ 0.125  \\ 
R76 & 6.631 $\pm$ 0.251 & 3.348 $\pm$ 0.167  \\ 
R77 & 8.194 $\pm$ 0.343 & 2.700 $\pm$ 0.131  \\ 
R78 & 7.981 $\pm$ 0.419 & 2.773 $\pm$ 0.094  \\ 
R79 & 6.794 $\pm$ 0.301 & 2.623 $\pm$ 0.082  \\ 
R80 & 7.454 $\pm$ 0.330 & 2.621 $\pm$ 0.093  \\ 
R81 & 7.236 $\pm$ 0.288 & 2.300 $\pm$ 0.109  \\ 
R83 & 7.441 $\pm$ 0.310 & 3.077 $\pm$ 0.109  \\ 
R84 & 7.582 $\pm$ 0.350 & 3.898 $\pm$ 0.371  \\ 
R85 & 7.359 $\pm$ 0.261 & 2.937 $\pm$ 0.110  \\ 
R86 & 7.711 $\pm$ 0.244 & 3.111 $\pm$ 0.109  \\ 
R87 & 7.025 $\pm$ 0.473 & 2.943 $\pm$ 0.105  \\ 
R88 & 8.033 $\pm$ 0.345 & 3.605 $\pm$ 0.184  \\ 
\hline

\end{longtable}
\begin{tablenotes}
\centering
\item $^a$ ($\lambda$8542\AA\ + $ \lambda$8662\AA + $ \lambda$8498\AA ). \\
\end{tablenotes}
\end{center}

==> Tables/TableEW_simple.tex <==
\begin{table}
\centering
\caption{Equivalent widths of stellar absorption lines of the observed CNSFRs. }
\label{tab:EW_MEGARA}
\begin{tabular}{ccc}
\hline
Region ID & \begin{tabular}[c]{@{}c@{}} EW(CaII)$^a$ \\ (\AA)\end{tabular} & \begin{tabular}[c]{@{}c@{}} EW(MgI) \\ (\AA)\end{tabular} \\
\hline
R1 & 7.307 $\pm$ 0.264 & 1.686 $\pm$ 0.035  \\ 
R3 & 7.301 $\pm$ 0.278 & 2.329 $\pm$ 0.063  \\ 
R4 & 7.558 $\pm$ 0.303 & 1.868 $\pm$ 0.044  \\ 
R5 & 7.418 $\pm$ 0.338 & 2.147 $\pm$ 0.048  \\ 
R6 & 7.118 $\pm$ 0.318 & 2.141 $\pm$ 0.073  \\ 
R7 & 6.732 $\pm$ 0.339 & 1.972 $\pm$ 0.056  \\ 
R8 & 7.350 $\pm$ 0.299 & 2.156 $\pm$ 0.060  \\ 
R9 & 7.571 $\pm$ 0.346 & 2.013 $\pm$ 0.054  \\ 
R10 & 7.008 $\pm$ 0.297 & 1.987 $\pm$ 0.048  \\ 
R11 & 7.281 $\pm$ 0.211 & 2.840 $\pm$ 0.092  \\ 
\hline
\end{tabular}
\tablefoot{$^a$($\lambda$8542\AA\ + $ \lambda$8662\AA + $ \lambda$8498\AA ). The complete table is available online; here only a part is shown as an example.
}

\end{table}

==> Tables/Vel_MEGARA.tex <==



\begin{center}
\begin{longtable}{llllll}
\caption{Emission line radial velocities in km/s.}
\hline
Region ID      & Component 
& \begin{tabular}[c]{@{}c@{}} v(H$\alpha$) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} v([NII]$\lambda$6584 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} v([SII]$\lambda$6717 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} v([SIII]$\lambda$9532 \AA) \\ (km/s)\end{tabular}
\\ \hline
\endfirsthead
\caption{continued.}\\
\hline
Region ID      & Component 
& \begin{tabular}[c]{@{}c@{}} v(H$\alpha$) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} v([NII]$\lambda$6584 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} v([SII]$\lambda$6717 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} v([SIII]$\lambda$9532 \AA) \\ (km/s)\end{tabular}
\\ \hline
\endhead
\hline
\endfoot

%%

R1 & Narrow & 8.45 $\pm$ 0.41 & 8.36 $\pm$ 8.52 & 6.80 $\pm$ 0.65 & 6.71 $\pm$ 1.71 \\
  & Broad & 5.48 $\pm$ 0.85 & 5.76 $\pm$ 12.02 & 7.00 $\pm$ 5.35 & 12.20 $\pm$ 9.46 \\ 
  & Aditional & 15.4 $\pm$ 1.2 & 12.86 $\pm$ 37.74 &  - &  - \\
\\
R3 & Narrow & 16.76 $\pm$ 0.09 & 16.57 $\pm$ 2.90 & 16.23 $\pm$ 0.58 & 15.42 $\pm$ 0.93 \\
  & Broad & 20.70 $\pm$ 0.95 & 18.72 $\pm$ 25.72 & 31.55 $\pm$ 9.52 &  - \\ 
\\
R4 & Narrow & 31.52 $\pm$ 0.20 & 32.54 $\pm$ 2.70 & 30.17 $\pm$ 1.12 & 30.07 $\pm$ 1.29 \\
  & Broad & 36.34 $\pm$ 0.78 & 36.35 $\pm$ 19.61 & 44.89 $\pm$ 5.20 &  - \\ 
  & Aditional & 18.2 $\pm$ 6.8 &  - &  - &  - \\
\\
R5 & Narrow & 26.16 $\pm$ 0.14 & 26.08 $\pm$ 2.50 & 24.49 $\pm$ 1.03 & 20.76 $\pm$ 0.71 \\
  & Broad & 8.65 $\pm$ 2.35 & 14.25 $\pm$ 2.81 &  - &  - \\ 
\\
R6 & Narrow & 29.24 $\pm$ 0.12 & 29.47 $\pm$ 1.50 & 30.00 $\pm$ 1.20 & 25.99 $\pm$ 0.73 \\
\\
R7 & Narrow & -1.17 $\pm$ 0.18 & -1.76 $\pm$ 2.25 & -5.16 $\pm$ 1.16 & -8.95 $\pm$ 1.11 \\
  & Broad & -11.31 $\pm$ 2.00 & -12.18 $\pm$ 34.27 &  - &  - \\ 
\\
R8 & Narrow & -12.66 $\pm$ 0.14 & -12.87 $\pm$ 2.25 & -15.13 $\pm$ 1.69 & -17.56 $\pm$ 1.10 \\
  & Broad & -20.15 $\pm$ 1.89 & -10.34 $\pm$ 1.99 &  - &  - \\ 
\\
R9 & Narrow & 20.77 $\pm$ 0.14 & 20.17 $\pm$ 1.74 & 16.97 $\pm$ 0.92 & 15.72 $\pm$ 0.86 \\
  & Broad & 17.62 $\pm$ 1.73 & 12.72 $\pm$ 4.85 &  - &  - \\ 
\\
R10 & Narrow & 13.33 $\pm$ 0.18 & 14.05 $\pm$ 2.75 & 10.04 $\pm$ 1.06 & 7.21 $\pm$ 1.32 \\
  & Broad & 12.28 $\pm$ 0.82 & 4.99 $\pm$ 2.79 &  - &  - \\ 
  & Aditional & 22.0 $\pm$ 3.7 &  - &  - &  - \\
\\
R11 & Narrow & -34.76 $\pm$ 0.13 & -35.52 $\pm$ 2.35 & -34.80 $\pm$ 1.11 & -28.15 $\pm$ 1.98 \\
  & Broad & -32.66 $\pm$ 0.67 & -32.13 $\pm$ 12.97 &  - &  - \\ 
\\
R12 & Narrow & 7.43 $\pm$ 0.20 & 7.75 $\pm$ 1.97 & 7.47 $\pm$ 1.11 & 0.42 $\pm$ 1.09 \\
  & Broad & 9.76 $\pm$ 1.08 & 13.28 $\pm$ 4.84 &  - &  - \\ 
\\
R14 & Narrow & 33.16 $\pm$ 0.57 & 33.19 $\pm$ 1.87 & 32.44 $\pm$ 1.08 & 29.22 $\pm$ 1.52 \\
  & Broad & 32.80 $\pm$ 0.83 & 27.62 $\pm$ 2.30 &  - &  - \\ 
\\
R15 & Narrow & 21.59 $\pm$ 0.20 & 21.20 $\pm$ 2.13 & 23.34 $\pm$ 1.25 & 19.14 $\pm$ 1.88 \\
  & Broad & 28.75 $\pm$ 2.27 & 29.54 $\pm$ 13.00 &  - &  - \\ 
\\
R16 & Narrow & 29.96 $\pm$ 0.11 & 29.77 $\pm$ 2.06 & 30.20 $\pm$ 0.71 & 34.24 $\pm$ 1.26 \\
  & Broad & 33.72 $\pm$ 0.96 & 33.29 $\pm$ 2.21 &  - &  - \\ 
\\
R17 & Narrow & 19.51 $\pm$ 0.48 & 19.75 $\pm$ 1.74 & 17.85 $\pm$ 1.08 & 18.66 $\pm$ 1.08 \\
  & Broad & 22.23 $\pm$ 2.07 & -2.46 $\pm$ 8.15 &  - &  - \\ 
  & Aditional & -5.6 $\pm$ 3.7 &  - &  - &  - \\
\\
R18 & Narrow & -32.03 $\pm$ 0.23 & -32.19 $\pm$ 2.36 & -33.38 $\pm$ 0.78 & -28.76 $\pm$ 1.11 \\
  & Broad & -32.32 $\pm$ 0.77 & -31.15 $\pm$ 13.14 &  - &  - \\ 
\\
R19 & Narrow & 24.30 $\pm$ 0.35 & 24.18 $\pm$ 2.95 & 24.44 $\pm$ 1.85 & 18.76 $\pm$ 1.95 \\
  & Broad & 27.52 $\pm$ 1.21 & 27.58 $\pm$ 18.10 &  - &  - \\ 
\\
R20 & Narrow & 22.41 $\pm$ 0.21 & 21.58 $\pm$ 1.66 & 18.83 $\pm$ 1.63 & 15.92 $\pm$ 1.32 \\
  & Broad & 20.35 $\pm$ 1.82 & 35.15 $\pm$ 4.77 &  - &  - \\ 
\\
R21 & Narrow & -22.03 $\pm$ 0.18 & -22.28 $\pm$ 1.93 & -22.68 $\pm$ 1.23 & -18.00 $\pm$ 2.02 \\
  & Broad & -21.05 $\pm$ 1.17 & -21.67 $\pm$ 18.40 &  - &  - \\ 
\\
R22 & Narrow & 5.10 $\pm$ 0.18 & 5.02 $\pm$ 2.09 & 8.86 $\pm$ 1.40 & 9.60 $\pm$ 1.40 \\
  & Broad & 10.42 $\pm$ 1.14 & 12.67 $\pm$ 21.81 &  - &  - \\ 
\\
R23 & Narrow & -32.87 $\pm$ 0.14 & -32.53 $\pm$ 2.16 & -32.46 $\pm$ 1.05 & -31.03 $\pm$ 2.33 \\
  & Broad & -28.32 $\pm$ 0.74 & -26.28 $\pm$ 21.73 &  - &  - \\ 
\\
R25 & Narrow & -6.54 $\pm$ 0.29 & -7.28 $\pm$ 2.03 & -8.44 $\pm$ 1.64 & -12.23 $\pm$ 1.95 \\
  & Broad & -8.81 $\pm$ 1.48 & -1.92 $\pm$ 36.18 &  - &  - \\ 
\\
R26 & Narrow & 2.20 $\pm$ 0.11 & 1.94 $\pm$ 2.83 & 2.88 $\pm$ 0.72 & 3.06 $\pm$ 1.21 \\
  & Broad & 2.15 $\pm$ 0.71 & 4.05 $\pm$ 14.49 &  - &  - \\ 
\\
R27 & Narrow & 36.94 $\pm$ 0.17 & 36.00 $\pm$ 1.65 & 40.85 $\pm$ 1.65 & 33.51 $\pm$ 1.38 \\
  & Broad & 34.07 $\pm$ 2.48 & 37.55 $\pm$ 3.81 &  - &  - \\ 
\\
R28 & Narrow & 11.51 $\pm$ 0.28 & 11.17 $\pm$ 2.75 & 9.57 $\pm$ 1.71 & 4.82 $\pm$ 2.29 \\
  & Broad & 7.78 $\pm$ 1.81 & 9.02 $\pm$ 3.04 &  - &  - \\ 
\\
R29 & Narrow & -14.42 $\pm$ 0.17 & -14.11 $\pm$ 1.97 & -11.46 $\pm$ 2.50 & -18.38 $\pm$ 1.61 \\
  & Broad & -11.40 $\pm$ 2.70 & -8.94 $\pm$ 3.24 &  - &  - \\ 
\\
R30 & Narrow & 18.25 $\pm$ 0.26 & 18.33 $\pm$ 1.90 & 18.33 $\pm$ 1.62 & 8.58 $\pm$ 1.60 \\
  & Broad & 18.49 $\pm$ 1.31 & 15.02 $\pm$ 12.76 &  - &  - \\ 
\\
R31 & Narrow & 36.84 $\pm$ 0.20 & 37.15 $\pm$ 1.84 & 37.46 $\pm$ 1.26 & 35.65 $\pm$ 3.19 \\
  & Broad & 40.23 $\pm$ 1.20 & 38.44 $\pm$ 18.80 &  - &  - \\ 
\\
R32 & Narrow & 22.39 $\pm$ 0.38 & 21.35 $\pm$ 1.92 & 20.17 $\pm$ 3.26 & 18.47 $\pm$ 3.59 \\
  & Broad & 13.25 $\pm$ 5.38 & 15.06 $\pm$ 23.31 &  - &  - \\ 
\\
R33 & Narrow & 36.32 $\pm$ 0.19 & 35.78 $\pm$ 1.82 & 34.69 $\pm$ 1.09 & 34.17 $\pm$ 1.60 \\
  & Broad & 34.71 $\pm$ 0.98 & 35.38 $\pm$ 13.34 &  - &  - \\ 
\\
R34 & Narrow & 3.65 $\pm$ 0.51 & 5.38 $\pm$ 4.40 & 4.42 $\pm$ 2.49 & 0.82 $\pm$ 1.80 \\
  & Broad & 8.36 $\pm$ 1.31 &  - &  - &  - \\ 
\\
R35 & Narrow & 2.89 $\pm$ 0.21 & 2.33 $\pm$ 1.86 & 2.10 $\pm$ 1.31 & 2.94 $\pm$ 1.64 \\
  & Broad & -0.14 $\pm$ 2.01 & -2.11 $\pm$ 19.32 &  - &  - \\ 
\\
R36 & Narrow & -25.79 $\pm$ 0.19 & -26.63 $\pm$ 2.51 & -24.12 $\pm$ 1.11 & -25.83 $\pm$ 2.17 \\
  & Broad & -23.90 $\pm$ 0.77 & -19.77 $\pm$ 16.98 &  - &  - \\ 
\\
R37 & Narrow & 24.90 $\pm$ 0.35 & 23.52 $\pm$ 2.03 & 14.58 $\pm$ 2.32 & 22.89 $\pm$ 2.69 \\
  & Broad & 13.91 $\pm$ 2.94 & 12.83 $\pm$ 19.68 &  - &  - \\ 
\\
R38 & Narrow & 36.11 $\pm$ 0.21 & 35.79 $\pm$ 3.00 & 34.75 $\pm$ 1.30 & 28.96 $\pm$ 1.73 \\
  & Broad & 36.86 $\pm$ 1.35 & 36.11 $\pm$ 4.37 &  - &  - \\ 
\\
R41 & Narrow & 34.67 $\pm$ 0.15 & 34.64 $\pm$ 1.92 & 35.04 $\pm$ 1.32 & 27.98 $\pm$ 2.33 \\
  & Broad & 33.56 $\pm$ 1.89 & 39.69 $\pm$ 32.18 &  - &  - \\ 
\\
R42 & Narrow & -32.40 $\pm$ 0.13 & -31.92 $\pm$ 2.04 & -32.07 $\pm$ 1.17 & -31.60 $\pm$ 1.69 \\
  & Broad & -31.31 $\pm$ 1.71 & -42.44 $\pm$ 4.57 &  - &  - \\ 
\\
R43 & Narrow & -8.73 $\pm$ 0.25 & -9.00 $\pm$ 1.87 & -10.08 $\pm$ 1.08 & -13.03 $\pm$ 2.53 \\
  & Broad & -3.94 $\pm$ 2.88 & -0.58 $\pm$ 31.93 &  - &  - \\ 
\\
R44 & Narrow & 35.03 $\pm$ 0.28 & 35.21 $\pm$ 2.17 & 35.13 $\pm$ 1.44 & 33.02 $\pm$ 4.99 \\
  & Broad & 30.09 $\pm$ 2.93 & 28.49 $\pm$ 12.51 &  - &  - \\ 
\\
R45 & Narrow & 24.60 $\pm$ 0.23 & 25.20 $\pm$ 2.35 & 27.57 $\pm$ 2.00 & 20.57 $\pm$ 6.19 \\
  & Broad & 23.16 $\pm$ 1.40 & 21.84 $\pm$ 18.15 &  - &  - \\ 
\\
R48 & Narrow & 39.32 $\pm$ 0.31 & 38.96 $\pm$ 2.31 & 40.78 $\pm$ 1.64 & 30.08 $\pm$ 4.62 \\
\\
R50 & Narrow & 15.98 $\pm$ 0.19 & 15.83 $\pm$ 2.77 & 16.41 $\pm$ 1.20 & 15.44 $\pm$ 1.51 \\
  & Broad & 15.36 $\pm$ 1.45 & 14.01 $\pm$ 17.63 &  - &  - \\ 
\\
R51 & Narrow & 2.94 $\pm$ 0.47 & 2.88 $\pm$ 2.97 & -0.77 $\pm$ 1.90 & -1.27 $\pm$ 2.43 \\
  & Broad & 3.98 $\pm$ 1.64 & 1.92 $\pm$ 8.11 &  - &  - \\ 
  & Aditional & 70.0 $\pm$ 5.1 &  - &  - &  - \\
\\
R52 & Narrow & -38.04 $\pm$ 0.23 & -37.78 $\pm$ 2.06 & -37.94 $\pm$ 1.26 &  - \\ 
  & Broad & -38.93 $\pm$ 0.94 & -30.11 $\pm$ 28.29 &  - &  - \\ 
\\
R53 & Narrow & 35.75 $\pm$ 0.31 & 34.68 $\pm$ 1.50 & 35.72 $\pm$ 1.28 & 32.18 $\pm$ 2.17 \\
  & Broad & 36.98 $\pm$ 1.76 & 43.82 $\pm$ 3.42 &  - &  - \\ 
\\
R54 & Narrow & 25.28 $\pm$ 0.52 & 24.02 $\pm$ 2.51 & 17.09 $\pm$ 1.89 & 17.19 $\pm$ 14.77 \\
  & Broad & 23.41 $\pm$ 1.46 & 25.02 $\pm$ 9.82 &  - &  - \\ 
\\
R55 & Narrow & 25.21 $\pm$ 0.34 & 25.25 $\pm$ 2.84 & 28.07 $\pm$ 1.47 & 28.46 $\pm$ 4.25 \\
  & Broad & 24.85 $\pm$ 1.70 &  - &  - &  - \\ 
\\
R56 & Narrow & -35.97 $\pm$ 0.25 & -36.12 $\pm$ 2.09 & -34.34 $\pm$ 1.73 & -36.20 $\pm$ 3.34 \\
  & Broad & -37.27 $\pm$ 1.38 & -39.26 $\pm$ 3.71 &  - &  - \\ 
\\
R57 & Narrow & -14.13 $\pm$ 0.33 & -13.65 $\pm$ 0.44 & -11.87 $\pm$ 1.73 & -8.81 $\pm$ 3.74 \\
  & Broad & -11.79 $\pm$ 1.38 &  - &  - &  - \\ 
\\
R58 & Narrow & -10.75 $\pm$ 0.46 & -11.11 $\pm$ 2.99 & -8.87 $\pm$ 1.48 & -11.74 $\pm$ 2.75 \\
  & Broad & -5.86 $\pm$ 1.47 & -8.30 $\pm$ 7.53 &  - &  - \\ 
\\
R59 & Narrow & 8.48 $\pm$ 0.80 & 6.90 $\pm$ 3.24 & 12.30 $\pm$ 1.46 & 13.59 $\pm$ 3.33 \\
  & Broad & 12.47 $\pm$ 1.39 & 16.39 $\pm$ 9.83 &  - &  - \\ 
\\
R60 & Narrow & -27.44 $\pm$ 1.13 & -29.83 $\pm$ 1.78 & -24.40 $\pm$ 2.44 &  - \\ 
  & Broad & -29.94 $\pm$ 1.72 & -25.08 $\pm$ 19.39 &  - &  - \\ 
  & Aditional & -23.1 $\pm$ 8.3 &  - &  - &  - \\
\\
R61 & Narrow & -18.37 $\pm$ 0.43 & -17.74 $\pm$ 1.89 & -25.36 $\pm$ 2.13 &  - \\ 
  & Broad & -23.49 $\pm$ 2.30 & -53.79 $\pm$ 8.01 &  - &  - \\ 
\\
R62 & Narrow & 9.08 $\pm$ 0.24 & 9.47 $\pm$ 1.85 & 5.95 $\pm$ 1.29 & -0.53 $\pm$ 2.26 \\
  & Broad & -21.94 $\pm$ 1.30 & -8.71 $\pm$ 4.24 &  - &  - \\ 
\\
R63 & Narrow & -23.16 $\pm$ 0.43 & -23.09 $\pm$ 0.02 & -23.19 $\pm$ 1.63 & -5.17 $\pm$ 8.10 \\
  & Broad & -27.74 $\pm$ 4.19 &  - &  - &  - \\ 
\\
R64 & Narrow & -28.54 $\pm$ 0.31 & -28.33 $\pm$ 2.00 & -30.42 $\pm$ 0.43 &  - \\ 
  & Broad & -29.32 $\pm$ 0.96 & -27.62 $\pm$ 18.21 &  - &  - \\ 
\\
R65 & Narrow & 22.12 $\pm$ 1.90 & 19.99 $\pm$ 3.36 & 15.27 $\pm$ 2.99 & 21.07 $\pm$ 6.32 \\
  & Broad & -11.48 $\pm$ 17.52 & 3.89 $\pm$ 20.36 &  - &  - \\ 
\\
R66 & Narrow & 2.72 $\pm$ 0.72 & -0.11 $\pm$ 3.34 & 2.49 $\pm$ 4.77 & - \\
  & Broad & -3.87 $\pm$ 9.61 &  - &  - &  - \\ 
\\
R67 & Narrow & -30.25 $\pm$ 0.57 & -31.57 $\pm$ 0.44 & -30.12 $\pm$ 2.88 & -35.77 $\pm$ 3.54 \\
  & Broad & -37.18 $\pm$ 2.95 &  - &  - &  - \\ 
  & Aditional & -30.3 $\pm$ 41.2 &  - &  - &  - \\
\\
R69 & Narrow & -37.75 $\pm$ 0.45 & -37.11 $\pm$ 0.44 & -36.20 $\pm$ 1.66 & -30.85 $\pm$ 4.43 \\
  & Broad & -37.30 $\pm$ 0.80 &  - &  - &  - \\ 
\\
R70 & Narrow & -27.76 $\pm$ 0.41 & -27.34 $\pm$ 0.44 & -19.86 $\pm$ 2.79 & -27.51 $\pm$ 4.44 \\
  & Broad & -25.25 $\pm$ 1.40 & -19.36 $\pm$ 0.44 &  - &  - \\ 
\\
R71 & Narrow & -23.83 $\pm$ 0.81 & -23.05 $\pm$ 2.16 & -25.74 $\pm$ 4.82 & 11.83 $\pm$ 8.24 \\
  & Broad & -12.49 $\pm$ 3.11 & -15.99 $\pm$ 5.19 &  - &  - \\ 
\\
R72 & Narrow & -9.06 $\pm$ 0.76 & -6.67 $\pm$ 2.36 & -3.37 $\pm$ 1.66 & 3.74 $\pm$ 9.92 \\
  & Broad & -13.21 $\pm$ 14.51 &  - &  - &  - \\ 
\\
R73 & Narrow & -4.25 $\pm$ 0.49 & -4.58 $\pm$ 1.71 & -0.47 $\pm$ 3.67 & 4.78 $\pm$ 5.77 \\
  & Broad & 3.05 $\pm$ 3.26 &  - &  - &  - \\ 
\\
R74 & Narrow & -26.39 $\pm$ 0.83 & -25.15 $\pm$ 4.40 & -20.34 $\pm$ 2.70 &  - \\ 
  & Broad & -23.90 $\pm$ 1.09 &  - &  - &  - \\ 
\\
R75 & Narrow & -36.09 $\pm$ 0.52 & -36.79 $\pm$ 2.43 & -37.62 $\pm$ 2.41 & -3.99 $\pm$ 10.24 \\
  & Broad & -39.62 $\pm$ 1.17 & -36.99 $\pm$ 9.10 &  - &  - \\ 
\\
R76 & Narrow & -36.02 $\pm$ 1.02 & -36.29 $\pm$ 0.44 &  - &  - \\ 
  & Broad & -36.20 $\pm$ 2.76 &  - &  - &  - \\ 
\\
R77 & Narrow & 32.96 $\pm$ 0.88 & 34.81 $\pm$ 2.80 & 32.86 $\pm$ 2.89 & 42.18 $\pm$ 6.19 \\
  & Broad & 45.81 $\pm$ 12.91 & 28.09 $\pm$ 17.70 &  - &  - \\ 
\\
R78 & Narrow & -34.01 $\pm$ 0.36 & -36.51 $\pm$ 2.98 & -30.98 $\pm$ 2.36 & -19.15 $\pm$ 5.50 \\
\\
R79 & Narrow & -38.11 $\pm$ 0.44 & -36.15 $\pm$ 2.73 & -42.11 $\pm$ 2.27 &  - \\ 
\\
R80 & Narrow & 36.02 $\pm$ 1.06 & 35.75 $\pm$ 3.72 & 34.29 $\pm$ 4.18 & 44.44 $\pm$ 11.54 \\
  & Broad & 23.15 $\pm$ 5.84 &  - &  - &  - \\ 
\\
R81 & Narrow & -33.21 $\pm$ 4.42 & -34.57 $\pm$ 1.97 & -32.45 $\pm$ 4.78 & -2.29 $\pm$ 9.84 \\
\\
R83 & Narrow & -31.66 $\pm$ 0.70 & -28.97 $\pm$ 2.22 & -30.74 $\pm$ 2.78 & -12.99 $\pm$ 12.92 \\
  & Broad & -28.34 $\pm$ 1.62 &  - &  - &  - \\ 
\\
R84 & Narrow & -24.83 $\pm$ 0.48 & -24.72 $\pm$ 2.17 & -19.45 $\pm$ 3.54 & -23.27 $\pm$ 6.79 \\
\\
R85 & Narrow & 40.32 $\pm$ 0.42 & 41.97 $\pm$ 2.35 & 44.65 $\pm$ 3.02 & 43.90 $\pm$ 4.47 \\
\\
R86 & Narrow & 38.53 $\pm$ 0.82 & 36.80 $\pm$ 2.58 & 33.48 $\pm$ 7.05 & 12.24 $\pm$ 9.29 \\
  & Broad & 42.41 $\pm$ 4.32 & 33.96 $\pm$ 9.17 &  - &  - \\ 
\\
R87 & Narrow & 32.97 $\pm$ 1.57 & 33.07 $\pm$ 2.41 &  - &  - \\ 
  & Broad & 37.86 $\pm$ 4.69 & 36.43 $\pm$ 8.65 &  - &  - \\ 
\\
R88 & Narrow & -14.69 $\pm$ 0.59 & -14.98 $\pm$ 2.47 & -4.36 $\pm$ 2.96 & 4.40 $\pm$ 6.90 \\
\end{longtable}
\end{center}





==> Tables/Vel_MEGARA_simple.tex <==
\begin{table*}
\centering
\caption{Emission line radial velocities in km/s.}
\label{tab:velocities_MEGARA}
\begin{tabular}{cccccc}
\hline
Region ID      & Component 
& \begin{tabular}[c]{@{}c@{}} v(H$\alpha$) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} v([NII]$\lambda$6584 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} v([SII]$\lambda$6717 \AA ) \\ (km/s)\end{tabular}
& \begin{tabular}[c]{@{}c@{}} v([SIII]$\lambda$9532 \AA) \\ (km/s)\end{tabular}
\\ \hline

R1 & Narrow & 8.45 $\pm$ 0.41 & 8.36 $\pm$ 8.52 & 6.80 $\pm$ 0.65 & 6.71 $\pm$ 1.71 \\
  & Broad & 5.48 $\pm$ 0.85 & 5.76 $\pm$ 12.02 & 7.00 $\pm$ 5.35 & 12.20 $\pm$ 9.46 \\ 
  & Aditional & 15.4 $\pm$ 1.2 & 12.86 $\pm$ 37.74 &  - &  - \\
\\
R3 & Narrow & 16.76 $\pm$ 0.09 & 16.57 $\pm$ 2.90 & 16.23 $\pm$ 0.58 & 15.42 $\pm$ 0.93 \\
  & Broad & 20.70 $\pm$ 0.95 & 18.72 $\pm$ 25.72 & 31.55 $\pm$ 9.52 &  - \\ 
\\
R4 & Narrow & 31.52 $\pm$ 0.20 & 32.54 $\pm$ 2.70 & 30.17 $\pm$ 1.12 & 30.07 $\pm$ 1.29 \\
  & Broad & 36.34 $\pm$ 0.78 & 36.35 $\pm$ 19.61 & 44.89 $\pm$ 5.20 &  - \\ 
  & Aditional & 18.2 $\pm$ 6.8 &  - &  - &  - \\

\hline


\end{tabular}

\tablefoot{
The complete table is available online; here only a part is shown as an example.
}
\end{table*}
